A Cornucopia of Carnot groups in Low Dimensions

Stratified groups are those simply connected Lie groups whose Lie algebras admit a derivation for which the eigenspace with eigenvalue 1 is Lie generating. When a stratified group is equipped with a left-invariant path distance that is homogeneous with respect to the automorphisms induced by the derivation, this metric space is known as Carnot group. Carnot groups appear in several mathematical contexts. To understand their algebraic structure, it is useful to study some examples explicitly. In this work, we provide a list of low-dimensional stratified groups, express their Lie product, and present a basis of left-invariant vector fields, together with their respective left-invariant 1-forms, a basis of right-invariant vector fields, and some other properties. We exhibit all stratified groups in dimension up to 7 and also study some free-nilpotent groups in dimension up to 14.

==> FreeGroups/Rank2Step6.tex <==
 

==> Parte_Finale.tex <==
  \section{Some free-nilpotent groups in low dimension}
ATTENZIONE: TUTTI I CONTI DI QUESTA SESSIONE VANNO CONTROLLATI

  \subsection{$\mathbb F_{r2}$}

  \subsection{$\mathbb F_{23}$}
\begin{example}
[The free nilpotent Lie algebra of rank $2$ and step $3$]
  
     A representation of the generators $X_{1},X_{2}$ as vector fields defined on $\mathbb{R}^{5}$ with respect to exponential coordinates of the second kind is the following:
  $$X_{1} = \partial_{1}$$ and  
\[
\begin{split}
X_{2} \ =\  &\partial_{2} -x_{1}\partial_{3} + \frac{x_{1}^{2}}{2}\partial_{4} + x_{1}x_{2}\partial_{5}.
\end{split}
\]
The other elements of the basis are the following: 
\[
\begin{split}
X_{3} \ =\  &\partial_3-  x_{1}\partial_{4} -x_{2}\partial_{5} ,
\end{split}\]
$$X_{4}=\partial_4, 
\qquad X_{5}=\partial_5 .$$

The bracket relations are:
$$X_3=[X_2,X_1],\;
X_4=[X_3,X_1],\;
X_5=[X_3,X_2].$$

 
 
 
 
 
The Baker-Campbell-Hausdorff formula for step-$3$ groups reads as
$$\exp X\exp Y= \exp\left(X + Y + \frac{1}{2}[X,Y] + \frac{1}{12}[X,[X,Y]] - \frac{1}{12}[Y,[X,Y]] \right).$$

Using the BCH formula, we compute the products in exponential coordinates of first kind:
$$\exp(a_1 X_1+\ldots+a_5 X_5)\cdot \exp(b_1 X_1+\ldots+b_5 X_5)=\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad $$
$$\qquad=
\exp\left( 
(a_1+b_1)  X_1+
(a_2+b_2) X_2+
(a_3+b_3+\dfrac{a_2b_1- a_1b_2}{2})  X_3 \right.\qquad\qquad$$ $$\qquad\qquad+
(a_4+b_4+ \dfrac{a_3b_1-a_1b_3}{2} + \dfrac{a_1(a_1b_2-a_2b_1)}{12} + \dfrac{b_1(a_2b_1-a_1b_2)}{12} )  X_4
$$ $$
\left.\qquad\qquad\qquad\qquad\qquad
+(a_5+b_5 + \dfrac{a_3b_2-a_2b_3}{2} - \dfrac{a_2(a_2b_1-a_1b_2)}{12} + \dfrac{b_2(a_2b_1-a_1b_2)}{12}   )  X_5\right)
$$

Using the BCH formula, we relates the  exponential coordinates of first kind to the exponential coordinates of second kind:
If $\alpha_1,\ldots, \alpha_5$ are the coordinates of second kind and
$a_1,\ldots, a_5$ are the coordinates of first kind,
then the change of coordinates are

NEED VERIFICATION!  see file Conti\_coordinate.pdf

%\begin{eqnarray*}
\begin{equation*}
\left\{\begin{array}{ccl}
a_1 &=&\alpha_1 \\
a_2 &=&\alpha_2\\
a_3 &=&\alpha_3+\dfrac{\alpha_1\alpha_2}{2}\\
a_4 &=&\alpha_4+\dfrac{\alpha_1\alpha_3}{2}+\dfrac{\alpha_1^2\alpha_2}{12}\\
a_5 &=&\alpha_5+\dfrac{\alpha_2\alpha_3}{2} - \dfrac{\alpha_1\alpha_2^2}{12},
\end{array}
\right.
\end{equation*}
%\end{eqnarray*}
\begin{equation*}
\left\{\begin{array}{ccl}
\alpha_1    &=&a_1\\
\alpha_2    &=&a_2\\
\alpha_3    &=&a_3 -\dfrac{1}{2} a_1 a_2\\
\alpha_4    &=&a_4 +\dfrac{1}{6} a_1^2 a_2 - \dfrac{1}{2} a_1 a_3\\
\alpha_5    &=&a_5+\dfrac{1}{3} a_1 a_2^2 - \dfrac{1}{2} a_2 a_3.
\end{array}
\right.
\end{equation*}
More explicitly, we have
$$
\exp(\alpha_5 X_5)\exp(\alpha_4 X_4)\cdot\ldots\cdot\exp(\alpha_1 X_1)=\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad$$
$$\qquad\quad=
\exp\left( \alpha_1 X_1+\alpha_2 X_2 + (\alpha_3+\dfrac{\alpha_1\alpha_2}{2})X_3 +(\alpha_4+\dfrac{\alpha_1\alpha_3}{2}+\dfrac{\alpha_1^2\alpha_2}{12})X_4+
(\alpha_5+\dfrac{\alpha_2\alpha_3}{2} - \dfrac{\alpha_1\alpha_2^2}{12}) X_5\right),$$
and viceversa
$$
\exp\left( a_1 X_1+a_2 X_2 + a_3 X_3 +a_4 X_4+a_5 X_5\right) 
=\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad$$
$$\qquad=
\exp((a_5 +\dfrac{1}{3} a_1 a_2^2 - \dfrac{1}{2} a_2 a_3) X_5 )\exp((a_4 +\dfrac{1}{6} a_1^2 a_2 - \dfrac{1}{2} a_1 a_3)  X_4)
\cdot\exp((a_3 -\dfrac{1}{2} a_1 a_2)X_3) 
\cdot\exp(a_2 X_2) \cdot\exp(a_1 X_1) $$


In exponential coordinates of second kind, the group law reads as
$$L_x(y)=x\cdot y=
(x_1+y_1, x_2+y_2,
x_3+y_3 -x_1y_2,
x_4+y_4 - x_1 y_3 +\frac{1}{2} x_1^2y_2,
x_5+y_5+x_1x_2y_2+\frac{1}{2}x_1y_2^2-x_2y_3)$$



\end{example}
  \subsection{$\mathbb F_{26}$}
\begin{example}[Rango 2 Step 6]  

The group is diffeomorphic to $\mathbb{R}^{23}$. In exponential coordinates, the first stratum is spanned by the two vectors: 
 \[
\begin{split}
X_{1} \ =\  &  \de_{1}
\\
X_{2} \ =\  &\de_{2} -x_{1}\de_{3} + \frac{x_{1}^{2}}{2}\de_{4} + x_{1}x_{2}\de_{5} - \frac{x_{1}^{3}}{6}\de_{6} - \frac{x_{1}^{2}x_{2}}{2}\de_{7} - \frac{x_{1}x_{2}^{2}}{2}\de_{8} \\ 
&~~~~ + \frac{x_{1}^{4}}{24}\de_{9} + \frac{x_{1}^{3}x_{2}}{6}\de_{10} + \frac{x_{1}^{2}x_{2}^{2}}{4}\de_{11} + \frac{x_{1}x_{2}^{3}}{6}\de_{12} - \frac{x_{1}^{2}x_{3}}{2}\de_{13} -x_{1}x_{2}x_{3}\de_{14}\\
&~~~~ - \frac{x_{1}^{5}}{120}\de_{15} 
- \frac{x_{1}^{4}x_{2}}{24}\de_{16} 
- \frac{x_{1}^{3}x_{2}^{2}}{12}\de_{17} 
- \frac{x_{1}^2x_{2}^{3}}{12}\de_{18} 
- \frac{x_{1}x_{2}^4}{24}\de_{19} \\ 
&~~~~ 
+  \frac{x_{1}^{3}x_{3}}{6}\de_{20}
+  \frac{x_{1}^{2}x_2 x_{3}}{2}\de_{21}
+  \frac{x_{1}x_2^{2}x_{3}}{2}\de_{22}
- x_{1}x_{2}x_{4}\de_{23}
.
\end{split}
\]
 The second stratum is one dimensional and generated by:
\[
\begin{split}
X_{3} \ =\  &\partial_3-  x_{1}\de_{4} -x_{2}\de_{5} + \frac{x_{1}^{2}}{2}\de_{6} +{x_{1}{}x_{2}}{}\de_{7} + \frac{x_{2}^{2}}{2}\de_{8} \\ 
&~~~~ - \frac{x_{1}^{3}}{6}\de_{9} - \frac{x_{1}^{2}x_{2}}{2}\de_{10} - \frac{x_{1}{}x_{2}^{2}}{2}\de_{11} - \frac{x_{2}^{3}}{6}\de_{12} +  {x_{1}{}x_{3}}{}\de_{13} +x_{2}x_{3}\de_{14},
 \\ 
&~~~~ + \frac{x_{1}^{4}}{24}\de_{15} 
+ \frac{x_{1}^{3}x_{2}}{6}\de_{16} 
+ \frac{x_{1}^{2}x_{2}^{2}}{4}\de_{17} 
+ \frac{x_{1}x_{2}^{3}}{6}\de_{18} 
+ \frac{x_{2}^4}{24}\de_{19} \\ 
&~~~~ 
-  \frac{x_{1}^{2}x_{3}}{2}\de_{20}
-  x_{1}x_2 x_{3}\de_{21}
-  \frac{x_2^{2}x_{3}}{2}\de_{22}
+ x_{2}x_{4}\de_{23}
.
\end{split}\]

Some brackets (not coming from Hall construction)
$$[X_1, X_{4}] = - X_{6}$$
$$[X_1, X_{5}] = - X_{7}$$
$$[X_1, X_{6}] = - X_{9}$$
$$[X_1, X_{7}] = - X_{10}-X_{13}$$
$$[X_1, X_{8}] = - X_{11}-X_{14}$$
$$[X_1, X_{9}] = - X_{15}$$
$$[X_1, X_{10}] = - X_{16}-X_{20}$$
$$[X_1, X_{11}] = - X_{17}-2X_{21}+X_{23}$$
$$[X_1, X_{12}] = - X_{18}-2X_{22}$$
$$[X_1, X_{13}] = - X_{20}$$
$$[X_1, X_{14}] = - X_{21}-X_{23}$$

$$[X_3, X_{4}] = - X_{13}$$
$$[X_3, X_{5}] = - X_{14}$$
$$[X_3, X_{6}] = - X_{20}$$
$$[X_3, X_{7}] = - X_{21}$$
$$[X_3, X_{8}] = - X_{22}$$
$$[X_4, X_{5}] = - X_{23}$$

\end{example}
  \subsection{$\mathbb F_{34}$}
\begin{example}[
The free, nilpotent Lie algebra of rank $3$ and step $4$]
The generators are $X_1, X_2, X_3$.
The brackets coming from the Hall basis are:
$$X_4 = [X_2,X_1], $$
$$X_5 = [X_3,X_1], $$
$$X_6 = [X_3,X_2], $$
$$X_7 = [X_4,X_1], $$
$$X_8 = [X_4,X_2], $$
$$X_9 = [X_4,X_3], $$
$$X_{10} = [X_5,X_1], $$
$$X_{11} = [X_5,X_2], $$
$$X_{12} = [X_5,X_3], $$
$$X_{13} = [X_6,X_2], $$
$$X_{14} = [X_6,X_3], $$
$$X_{15} =... $$
...
$$X_{32} =... $$


Some brackets (not coming from Hall construction)
$$[X_1, X_{6}] =  X_{9}-X_{11}$$
 $$[X_1, X_{8}] = - X_{16} $$
$$[X_1, X_{9}] = -X_{17}+X_{30}$$
$$[X_1, X_{11}] = - X_{22}- X_{30}$$
$$[X_1, X_{12}] = - X_{23}$$
$$[X_1, X_{13}] = X_{19}-X_{24}-2 X_{31}$$
$$[X_1, X_{14}] = X_{20}-X_{25}-X_{32}$$

$$[X_9, X_{2}] = X_{19}- X_{31}$$
$$[X_9, X_{3}] = X_{20} $$

$$[X_2, X_{12}] = X_{32}-X_{25}$$
$$[X_2, X_{14}] =  -X_{28} $$


The group is diffeomorphic to $\mathbb{R}^{32}$. In exponential coordinates of type $2$, the horizontal distribution is spanned by the three vector fields: 
 \[
\begin{split}
X_{1} \ =\  &  \de_{1},
\\
X_{2} \ =\  &\de_{2} -x_{1}\de_{4} + \frac{x_{1}^{2}}{2}\de_{7} + x_{1}x_{2}\de_{8} 
+ x_{1}x_{3}\de_{9}
 \\
&~~~~~~~~
- \frac{x_{1}^{3}}{6}\de_{15}
 - \frac{x_{1}^{2}x_{2}}{2}\de_{16} 
 - \frac{x_{1}^{2}x_{3}}{2}\de_{17} 
 - \frac{x_{1}x_{2}^{2}}{2}\de_{18} 
 -x_1 x_2 x_3 \de_{19} 
 - \frac{x_{1}x_{3}^{2}}{2}\de_{20} 
,
\end{split}
\] 

 \[
\begin{split}
X_{3} \ =\  &  \de_{3}  
-x_{1}\de_{5} 
-x_{2}\de_{6} 
+ \frac{x_{1}^{2}}{2}\de_{10}
 + x_{1}x_{2}\de_{11} 
 + x_{1}x_{3}\de_{12} 
 + \frac{x_{2}^{2}}{2}\de_{13}
  + x_{2}x_{3}\de_{14} 
  \\
&~~~~~~~~
 - \frac{x_{1}^{3}}{6}\de_{21}
 - \frac{x_{1}^{2} x_2}{2}\de_{22}
 - \frac{x_{1}^{2} x_3}{2}\de_{23}
 - \frac{x_{1} x_2^{2}}{2}\de_{24}
 - x_{1}x_2 x_{3}\de_{25}
   - \frac{x_{1} x_3^{2}}{2}\de_{26}
   \\
&~~~~~~~~
    - \frac{x_{2}^{3}}{6}\de_{27}
 - \frac{x_{2}^{2} x_3}{2}\de_{28}
 - \frac{x_{2}x_3^{2} }{2}\de_{29}
 + x_{1}x_{4}\de_{30} 
 + x_{2}x_{4}\de_{31} 
 + x_{2}x_{5}\de_{32} .
\end{split}
\] 

\end{example}
  \subsection{$\mathbb F_{25}$}
\begin{example}[
The free, nilpotent Lie algebra of rank $2$ and step $5$]
The generators are $E_1, E_2$.
The brackets coming from the Hall basis are:
$$E_3 = [E_2,E_1], $$
$$E_4 =[E_3,E_1], E_5 = [E_3,E_2], $$
$$E_6 = [E_4,E_1], E_7 = [E_4,E_2], E_8 = [E_5,E_2], $$
$$E_9 =[E_6,E_1], E_{10} = [E_6,E_2], E_{11} = [E_7,E_2], E_{12} = [E_8,E_2], E_{13} = [E_4,E_3],
E_{14} = [E_5,E_3],$$
All the other brackets with respect to the generators are 
$$[E_5,E_1]=E_7,$$
$$[E_7,E_1]=E_{10}+E_{13},$$
$$[E_8,E_1]=E_{11}+E_{14}.$$



A representation of the generators $E_{1},E_{2}$ as vector fields defined on $\mathbb{R}^{14}$ with respect to exponential coordinates of the second kind is $E_{1} = \de_{1}$ and 
\[
\begin{split}
E_{2} \ =\  &\de_{2} -x_{1}\de_{3} + \frac{x_{1}^{2}}{2}\de_{4} + x_{1}x_{2}\de_{5} - \frac{x_{1}^{3}}{6}\de_{6} - \frac{x_{1}^{2}x_{2}}{2}\de_{7} - \frac{x_{1}x_{2}^{2}}{2}\de_{8} \\ 
&~~~~ + \frac{x_{1}^{4}}{24}\de_{9} + \frac{x_{1}^{3}x_{2}}{6}\de_{10} + \frac{x_{1}^{2}x_{2}^{2}}{4}\de_{11} + \frac{x_{1}x_{2}^{3}}{6}\de_{12} - \frac{x_{1}^{2}x_{3}}{2}\de_{13} -x_{1}x_{2}x_{3}\de_{14}.
\end{split}
\]
The other elements of the basis are the following: 
\[
\begin{split}
E_{3} \ =\  &\partial_3-  x_{1}\de_{4} -x_{2}\de_{5} + \frac{x_{1}^{2}}{2}\de_{6} +{x_{1}{}x_{2}}{}\de_{7} + \frac{x_{2}^{2}}{2}\de_{8} \\ 
&~~~~ - \frac{x_{1}^{3}}{6}\de_{9} - \frac{x_{1}^{2}x_{2}}{2}\de_{10} - \frac{x_{1}{}x_{2}^{2}}{2}\de_{11} - \frac{x_{2}^{3}}{6}\de_{12} +  {x_{1}{}x_{3}}{}\de_{13} +x_{2}x_{3}\de_{14},
\end{split}\]
$$E_{4}=\partial_4-x_1\partial_6-x_2\partial_7 +\dfrac{x_1^2}{2}\partial_{9}+x_1x_2 \partial_{10}+\dfrac{x_2^2}{2}\partial_{11}-x_3\partial_{13,}$$
$$E_{5}=\partial_5 -x_1\partial_7-x_2\partial_8+\dfrac{x_1^2}{2}\partial_{10} +x_1x_2\partial_{11} +\dfrac{x_2^2}{2}\partial_{12} -x_3\partial_{14}+ \dfrac{x_1^2}{2}\partial_{13} ,$$
$$E_{6}=\partial_6 -x_1\partial_9-x_2\partial_{10},$$
$$E_{7}=\partial_7 - x_1\partial_{10}-x_2\partial_{11}-x_1\partial_{13},$$
$$E_{8}=\partial_8 - x_1\partial_{11}-x_2\partial_{12}-x_1\partial_{14},$$
$$E_{9}=\partial_9,$$
$$E_{10}=\partial_{10},$$
$$E_{11}=\partial_{11},$$
$$E_{12 }=\partial_{12}, $$
$$E_{13}=\partial_{13},$$
$$E_{14}=\partial_{14}.$$

\end{example}

